Tangent: An Empirical Study of Testing Practices for LLM-Based Agent Applications

Agents built on large language models (LLMs) are increasingly used to build applications that perform complex, multi-step tasks involving reasoning, tool use, and interaction with external environments. Despite rapid progress in benchmarking LLM-based agents, very few studies have attempted to understand how such systems are tested in practice. In particular, testing levels, objectives, data patterns, test complexity, and validation strategies for agent applications remain underexplored. In this paper, we present an empirical study of testing practices in LLM-based agent applications using a large corpus of mined open-source projects. We construct a large-scale dataset of agent applications, tools, and tests, and manually label 2,572 test methods from 240 modules. From this analysis, we derive a taxonomy of 23 testing patterns across test fixtures, data, objectives, and assertions, and characterize tests by level (unit, module, integration). We complement this with structured interviews of 10 senior industry practitioners building agentic systems. Our results show that testing of LLM-based agent applications is dominated by narrowly scoped unit tests, with limited coverage of complex interactions, realistic scenarios, and non-functional requirements. Tests frequently rely on simplistic inputs, heavy mocking, and shallow validation, and agent-related tests exhibit low structural complexity. While industry practice places greater emphasis on non-functional testing than open-source projects, both reveal common gaps, including the lack of formal testing foundations, unclear test objectives, and challenges in generating high-quality test data. Based on these findings, we outline research directions toward more systematic and rigorous testing of agent applications, including foundations for agent testability, formalized test objectives, and fault-based testing techniques.

==> cacm.tex <==
\section{Challenges in Testing Agents}
\label{sec:challenges}

Testing LLM-based agent applications introduces challenges that go beyond those encountered in conventional software testing. These challenges stem from the defining properties of agentic systems: stochastic behavior, multi-step reasoning, tool use, interaction with external environments, and emergent behavior over long execution horizons. Together, these properties complicate how developers define correctness, observe failures, measure coverage, and automate regression testing. In this section, we summarize the key challenges that arise when testing agentic systems.

\subsection{Test Oracle Problem}
\label{subsec:oracle}

The test oracle problem---determining whether an observed behavior is correct---is especially acute in LLM-based agent applications. In conventional software, testers can often specify an expected output for a fixed input and compare the observed result against it. In agentic systems, however, correctness is often \emph{distributional rather than point-valued}. The same query may produce different, yet equally acceptable, responses across executions. Acceptability may also depend on context, phrasing, intermediate reasoning paths, and the persona or role of the end user, such as a product manager versus a technical lead. As a result, assertions must be flexible enough to admit legitimate variation while still being precise enough to detect real failures.


\subsection{Testing Non-deterministic Behavior}
\label{subsec:nondeterminism}

Non-determinism is one of the most fundamental obstacles to reliable agent testing. Because LLM inference is stochastic, repeated executions of the same test may produce different final outputs, intermediate tool calls, or reasoning paths. This undermines traditional testing assumptions, where a fixed input is expected to produce a fixed and reproducible output. A test may pass in one run and fail in another without any change to the system under test, producing behavior analogous to flaky tests in conventional software~\cite{dutta2020detecting, rahman2025understanding}.

Non-determinism also complicates debugging and test isolation. When a failure occurs, developers may be unable to determine whether it reflects a genuine defect, a sampling artifact, an environmental condition, or an interaction among these factors. Reproducing failures requires controlling, replaying, or at least logging the stochastic elements of execution, but current testing frameworks provide limited support for doing so across the full agentic stack.

Several approaches from software testing offer useful foundations. Property-based testing~\cite{hughes2007quickcheck} and metamorphic testing~\cite{chen1998metamorphic} shift the focus from exact output equivalence to relational properties that should hold across executions. Techniques from probabilistic program testing~\cite{dutta2018testing, borges2015iterative, luckow2014exact} and model checking~\cite{mardziel2013dynamic, monniaux2000abstract} provide formal foundations for reasoning about stochastic systems. Recent work has begun adapting these ideas to agents: ToolFuzz~\cite{milev2025toolfuzz} fuzzes tool runtimes, ChainFuzzer~\cite{wu2026chainfuzzer} targets multi-tool workflows, and agentic property-based testing~\cite{maaz2025agentic} explores bug finding across LLM-powered components. However, a comprehensive framework for managing non-determinism across prompts, models, tools, memory, and external environments remains absent.

\subsection{Testing Trajectories}
\label{subsec:trajectories}

Agent behavior is not fully captured by final outputs. Many failures arise from the \emph{trajectory} of execution: the sequence of reasoning steps, tool selections, delegation decisions, intermediate states, and environment transitions that lead to a final result. Testing these trajectories is therefore one of the most distinctive challenges in agent testing.

Observability platforms such as LangSmith~\cite{langchain2026trajectory}, LangFuse~\cite{langfuse2025}, Arize AI~\cite{arize2026}, and Maxim AI~\cite{maximai2026} expose execution traces, intermediate decisions, tool calls, and environment transitions. However, these artifacts are typically external to the main test suite and are not well integrated with standard testing frameworks such as PyTest and Unittest. Consequently, even when developers inspect trajectories during debugging, those checks are rarely encoded as automated, reusable assertions. This creates a gap between what can be observed and what is systematically validated during routine development.

Bridging this gap requires testing infrastructure that supports first-class assertions over trajectories, including tool-selection paths, delegation patterns, reasoning traces, and multi-step task execution~\cite{kim2025beyond, qian2025webgrapheval}. Such assertions may need to operate at different levels of granularity: individual tool calls, subtask plans, full execution traces, or resulting environment states. Formalizing what constitutes an acceptable trajectory, and defining adequacy criteria based on trajectory coverage rather than only code coverage, remain important open problems.

\subsection{Testing Non-functional Requirements}
\label{subsec:nfr}

Non-functional requirements (NFRs)---including security, performance, resilience, privacy, and policy compliance---are critical for agentic systems because agents increasingly interact with external tools, sensitive data, and real-world environments. Yet NFR testing remains underrepresented in practice. Empirical evidence from open-source agent projects~\cite{pan2026tangent} shows that only a small fraction of tests, roughly 7--8\%, target NFRs at all. Among those tests, most focus on security scenarios, while performance, memory, and resilience receive substantially less attention.

This scarcity reflects several compounding difficulties. Performance and latency are difficult to evaluate without realistic workloads and deployed environments, which are often unavailable during unit testing. Security properties, such as prompt-injection resistance, PII anonymization, and privilege-escalation prevention, require adversarial inputs that are difficult to construct systematically. Resilience testing, which evaluates behavior under partial failures such as tool timeouts, schema drift, or unreachable services, requires fault-injection capabilities that current agent frameworks rarely expose.

Established software engineering techniques provide a useful starting point. Fault injection~\cite{arlat1990fault, segall1995fiat}, chaos engineering~\cite{basiri2016chaos}, and metamorphic testing~\cite{chen2018metamorphic} are well-established approaches for evaluating behavior under failures and adversarial conditions. Recent work has begun extending these approaches to agents: MAST~\cite{cemri2026multi} catalogs behavioral failure modes in multi-agent execution traces, ReliabilityBench~\cite{gupta2026reliabilitybench} applies chaos engineering to single-agent systems using infrastructure-level faults, and MAS-FIRE~\cite{jia2026masfire} defines a fault taxonomy for multi-agent systems. However, prior work has not yet provided a unified fault taxonomy or injection mechanism that spans the full agentic stack, including tool integration, memory, inter-agent communication, security, and fault propagation across architectural layers.

\subsection{End-to-end Testing}
\label{subsec:e2e}

End-to-end (E2E) testing exercises a complete flow from user input through all system layers to the final outcome. For agentic systems, E2E testing is especially important because correctness often depends on the composition of agents, tools, memory, external services, and environment side effects across a full task. At the same time, E2E testing is difficult to perform in practice. It typically requires a deployed or near-deployed environment, realistic user inputs, and mechanisms for observing and asserting on outcomes that may span multiple turns, tool invocations, and external state changes.

A central difficulty is distinguishing integration testing from true E2E testing when the application is not fully deployed. E2E tests also face the full force of the oracle problem (Section~\ref{subsec:oracle}) and non-determinism (Section~\ref{subsec:nondeterminism}), because both are amplified when the entire system is exercised together. Validating environment side effects, such as files written, database entries modified, or external services called, adds further complexity.

Recent benchmarks such as $\tau$-bench~\cite{yao2024taubench} and OSWorld~\cite{xie2024osworld} move toward E2E evaluation by assessing resulting system state rather than only final outputs. However, systematic support for E2E testing of agent workflows in development settings remains limited. Developers still lack practical tools for constructing realistic scenarios, controlling external dependencies, validating side effects, and replaying failures with sufficient determinism for regression testing.

\subsection{Test Adequacy Metrics}
\label{subsec:adequacy}

Measuring the adequacy of a test suite---how much of the system has been exercised and how well---is a long-standing concern in software testing. Conventional criteria such as statement coverage, branch coverage, and mutation score provide well-defined measures for traditional software~\cite{ammann2016introduction, zhu1997software, jia2011mutation, weyuker1988evaluating}. These criteria, however, do not capture the higher-level abstractions that characterize agentic systems, including tool-selection paths, reasoning traces, delegation patterns, multi-step task execution, memory interactions, and environment state transitions.

In practice, no widely accepted adequacy standard exists for agent testing. Practitioners instead rely on ad hoc approaches such as edge-case coverage, domain-driven test design, trajectory sampling, query clustering, and acceptable failure thresholds---all of which are project-specific judgments rather than formal criteria~\cite{pan2026tangent}. This creates uncertainty about when a test suite is sufficiently comprehensive and makes it difficult to compare testing practices across projects.

Developing adequacy metrics for agentic systems likely requires moving beyond code coverage toward behavioral and interaction coverage. Examples include coverage over tool-use patterns, prompt and input distributions, execution trajectories, memory states, delegation structures, and environment-side effects. These metrics must also account for stochastic behavior, since a single execution may not adequately characterize an agent's behavior under a given scenario.

\subsection{Agent-specific Test Frameworks}
\label{subsec:framework}

Despite the rapid growth of LLM-based agent applications, the tooling and infrastructure for testing them remain immature. General-purpose frameworks such as PyTest and Unittest were designed for conventional software and do not natively support assertions over execution trajectories, delegation behavior, reasoning steps, non-deterministic outputs, or environment side effects. Although observability platforms expose many of these artifacts, they are often separate from the test suite and are not designed for automated, regression-style validation.

Agent-specific test infrastructure is therefore needed to treat trajectories, tool calls, intermediate reasoning states, memory interactions, and environment transitions as first-class test targets. Such infrastructure should provide: (1) reusable test doubles that simulate not only tool execution behavior but also the effects of tool descriptions on agent reasoning~\cite{hasan2026mcp}; (2) distributional assertions for validating stochastic behavior across repeated executions; (3) mechanisms for replaying execution traces with sufficient determinism for regression testing; and (4) integration with observability data so that trajectory-level assertions can be embedded within standard testing workflows. Developing this infrastructure, grounded in a rigorous theory of agent testability that extends classical notions of controllability and observability~\cite{freedman1991testability, voas2002testability} to the agentic setting, is a key prerequisite for systematic and rigorous testing of LLM-based agent applications.


==> rq1_agent.tex <==
\section{Agent Statistics}
\label{sec:rq_agent_statistics}
% Before we understand the testing practices in the LLM-based agentic applications, we want to understand how complex these agents are, what kind of framework do developers use, how complex the codebase in terms of structural complexity including number of line of code, number of application, library calls, etc. Below we discuss each.
Before discussing the testing practices used in LLM-based agentic applications, we first examine how complex these agents are, which frameworks developers use, and the structural complexity of the codebases, including the number of lines of code and the number of application and library calls. Below, we discuss each of these aspects.

\paragraph{Distribution by Framework}
\begin{figure}[!htp]
    \centering
    \includegraphics[width=\columnwidth]{figures/fig1_agents_tools_by_framework.pdf}
    \caption{Agents and tools by framework.}
    \label{fig:fig1_agents_tools_by_framework}
\end{figure}

Figure~\ref{fig:fig1_agents_tools_by_framework} presents the distribution of agent and tool frameworks used across the analyzed systems. In terms of agent development, LangGraph and AutoGen are the most commonly used frameworks for building agentic architectures, followed by LangChain and the OpenAI Agent SDK.
For tool development, LangChain, Model Context Protocol (MCP), and FastMCP appear as the most prevalent frameworks. Notably, MCP and FastMCP are specifically designed to support tool integration by exposing tools as distributed services. This design enables agents or LLMs to dynamically discover and invoke tools as needed, allowing solutions to be constructed on demand.
In contrast, agent frameworks typically introduce clearer structural boundaries. Each agent is responsible for performing a specific task and interacts with a sequence of tools to complete its assigned action. This structured design supports coordinated workflows while maintaining well-defined responsibilities for each agent within the system. For instance, .... \rangeet{have one example of a series of tools loaded to an MCP server and one for an agent with several tools, and discuss how testing them will be completely different.}
\paragraph{Structural Complexity}
\begin{itemize}[leftmargin=*]
    \item \textbf{Application Calls.}
    \item \textbf{Constructor Calls.}
    \item \textbf{Library Calls.}
    \item \textbf{Cyclomatic Complexity.}
    \item \textbf{NCLOC.}
\end{itemize}

\begin{figure*}[!t]
    \centering
    
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig2_application_calls_by_framework.pdf}
        \caption{Application Calls}
        \label{fig:fig2_application_calls}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig2_constructor_calls_by_framework.pdf}
        \caption{Constructor Calls}
        \label{fig:fig2_constructor_calls}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig2_library_calls_by_framework.pdf}
        \caption{Library Calls}
        \label{fig:fig2_library_calls}
    \end{subfigure}
    
    \caption{Agents Calls By Frameworks: (a) Application Calls, (b) Constructor Calls, and (c) Library Calls.}
    \label{fig:fig2_combined}
\end{figure*}

\begin{figure*}[!htp]
    \centering
    
    % \begin{minipage}[b]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/fig2b_overall_agent_complexity.pdf}
    %     \caption*{(a) Overall}
    % \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig2_cyclomatic_complexity_by_framework.pdf}
        \caption*{(b) Cyclomatic}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig2_ncloc_by_framework.pdf}
        \caption*{(c) NCLOC}
    \end{minipage}
    
    \caption{Agents Complexity Metrics: (a) Overall Complexity, (b) Cyclomatic Complexity by Frameworks, and (c) NCLOC by Frameworks.}
    \label{fig:fig2_complexity_combined}
\end{figure*}

\paragraph{Future Research Directions}

==> rq2_agent_test_statistics.tex <==
\section{Agent Specific Test Statistics}
\label{sec:rq_agent_test_statistics}

\paragraph{Future Research Directions}

==> tables/agents_tools.tex <==
\begin{wraptable}{r}{0.42\linewidth}
\vspace{-5pt}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\caption{Distribution of frameworks used for building agents and tools.}
\begin{tabular}{lrr}
\hline
Framework & Agents & Tools \\
\hline
LangChain         & 224 & 860 \\
MCP               &   0 & 695 \\
AutoGen           & 348 &  41 \\
CrewAI            & 191 & 190 \\
OpenAI Agents SDK & 222 & 147 \\
FastMCP           &   0 & 359 \\
LangGraph         & 356 &   1 \\
Swarm             &  44 &  15 \\
LlamaIndex        &   1 &   4 \\
Semantic Kernel   &   0 &   2 \\
Letta             &   1 &   0 \\
\hline
\end{tabular}
\label{tb:agents}
\vspace{-10pt}
\end{wraptable}
